Formalizing Mathematics at Scale

We present AutoformBot, a multi-agent system for building an Autoformalized Textbook Library At Scale (Atlas) in Lean 4. AutoformBot orchestrates thousands of LLM agents, equipped with formal verification tools, dependency-aware task scheduling, and collaborative version control, to translate informal textbook prose into machine-checked definitions and proofs. We apply our methods to a corpus of 26 open-access textbooks spanning analysis, algebra, topology, combinatorics, and probability, producing Atlas: a verified library of over 45,000 Lean 4 declarations and 500 thousand lines of code. We release two artifacts: (i) AutoformBot, the open-source multi-agent framework; and (ii) Atlas, the resulting formal library. Our results suggest that autoformalizing the core content of graduate-level mathematics at scale is now economically and technically feasible. This opens the door to the automated verification of both human- and machine-generated mathematics at a research level.

==> template/dark.tex <==

\usepackage{xcolor}
\definecolor{coolblack}{RGB}{40, 40, 45}
\definecolor{coolwhite}{RGB}{160, 160, 160}
\definecolor{coolblue}{RGB}{65, 130, 205}
\pagecolor{coolblack}
\color{coolwhite}   
\PassOptionsToPackage{allbordercolors=coolblue,allcolors=coolblue,colorlinks=true}{hyperref}
\definecolor{coolred}{RGB}{200, 60, 100}
\renewcommand\note[1]{{\color{coolred} #1}}


==> template/package.tex <==
%%%% Packages

%% Encoding
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

%% Fonts — skip when fairmeta supplies its own
\makeatletter
\@ifclassloaded{fairmeta}{}{%
  \usepackage{times}
}
\makeatother

%% Links
\PassOptionsToPackage{hyphens}{url}
\usepackage{url}
\usepackage{hyperref}

%% Graphics
\usepackage{graphicx}
\usepackage{caption}
\makeatletter
\@ifclassloaded{fairmeta}{}{%
  \captionsetup{margin=10pt,font=small,labelfont=bf}
}
\makeatother
\usepackage{tikz}
\usetikzlibrary{positioning,shapes.geometric,calc}
\usepackage{pgfplots}
\pgfplotsset{compat=1.17}

%% Essentials

% Rendering enhancement
\usepackage{array}
\usepackage{booktabs}
\usepackage{microtype}
% Color
\usepackage{xcolor}
% Float
\usepackage{float}
% Itemize
\IfFileExists{enumitem.sty}{
  \usepackage{enumitem}
  \setitemize{itemsep=0pt,parsep=0pt,topsep=0pt}
  \setenumerate{itemsep=0pt,parsep=0pt,topsep=0pt}
}{}

% Algorithmic package
\IfFileExists{algorithm.sty}{
  \usepackage{algorithm}
  \usepackage{algorithmicx}
  \usepackage{algpseudocode}
}{}

%% Code listings (Lean 4)
\usepackage{listings}
\lstdefinestyle{lean}{
  basicstyle=\ttfamily\small,
  breaklines=true,
  columns=fullflexible,
  keepspaces=true,
  xleftmargin=4pt,
  aboveskip=6pt,
  belowskip=6pt,
  literate=
    {ℝ}{{$\mathbb{R}$}}1
    {ℕ}{{$\mathbb{N}$}}1
    {→}{{$\to$}}1
    {←}{{$\leftarrow$}}1
    {∀}{{$\forall$}}1
    {∃}{{$\exists$}}1
    {≤}{{$\le$}}1
    {≥}{{$\ge$}}1
    {≠}{{$\ne$}}1
    {⊆}{{$\subseteq$}}1
    {∈}{{$\in$}}1
    {∉}{{$\notin$}}1
    {⁻¹}{{$^{-1}$}}1
    {∫}{{$\int$}}1
    {α}{{$\alpha$}}1
    {·}{{$\cdot$}}1
    {⟩}{{$\rangle$}}1
    {⟨}{{$\langle$}}1
}
\lstset{style=lean}

%% Natbib bibliography
\usepackage{natbib}

%% To edit with several authors
\usepackage[normalem]{ulem}

% Bookcards

%% Per-book result cards (colored boxes in the per-book appendix)
\usepackage[most]{tcolorbox}
\newtcolorbox{bookcardbox}[1][]{%
  enhanced,
  breakable,
  colback=green!5!white,
  colframe=green!45!black,
  colbacktitle=green!18!white,
  coltitle=green!30!black,
  fonttitle=\bfseries,
  title filled,
  arc=6pt,
  boxrule=0.6pt,
  left=8pt,right=8pt,top=5pt,bottom=5pt,
  toptitle=3pt,bottomtitle=3pt,
  #1
}
% \bookcard{Title}{Author}{URL}{Targets}{Pages}{LoC}{Formalized}{Gaps}{Tokens}{Comments}
% (split in two stages because TeX macros are limited to 9 args)
\makeatletter
\newcommand{\bookcard}[2]{%
  \def\bk@title{#1}\def\bk@author{#2}\bookcard@aux
}
\newcommand{\bookcard@aux}[8]{%
  \begin{bookcardbox}[title={\emph{\bk@title}, by \bk@author}]
    \footnotesize
    \setlength{\extrarowheight}{2pt}%
    {\sloppy\raggedright\href{#1}{\nolinkurl{#1}}\par}\smallskip
    \begin{tabular}{@{}p{0.30\linewidth}p{0.36\linewidth}p{0.30\linewidth}@{}}
      \textbf{Target statements:} #2 &
      \textbf{Formalized statements:} #5 &
      \\
      \textbf{Pages:} #3 &
      \textbf{Lines of code:} #4 &
      \textbf{Tokens (M):} #7 \\
    \end{tabular}\par\smallskip
  \end{bookcardbox}%
}
\makeatother

